Uncovering Plagiarism Networks

Plagiarism detection in educational programming assignments is still a problematic issue in terms of resource waste, ethical controversy, legal risks, and technical complexity. This paper presents AC, a modular plagiarism detection system. The design is portable across platforms and assignment formats and provides easy extraction into the internal assignment representation. Multiple similarity measures have been incorporated, both existing and newly-developed. Statistical analysis and several graphical visualizations aid in the interpretation of analysis results. The system has been evaluated with a survey that encompasses several academic semesters of use at the authors' institution.

==> outliers.tex <==
\subsection{Threshold recommendation and outlier detection}
\label{outliers}

The result of performing similarity calculations is a large (quadratic in the number of submission in the corpus) number of pairwise distances, a number of which will be very low in case of plagiarism occurrence. The goal
of a plagiarism detection tool is to flag these distances as suspicious. A
human grader can then locate cases of plagiarism by visual inspection of only the (few) likely candidates, without requiring analysis of the remaining set of (many) non-plagiarized pairs.

When based only on either the bulk of distance values, the process of
flagging likely candidates depends on the determination of a
\emph{similarity threshold} value. If a pair of submission has a
similarity distances which falls below this threshold, it will be
flagged for inspection. Otherwise, the pair will not be flagged. Of
course, the use of a single threshold value incurs the risk of false
positives and false negatives. Graders should be aware of these risks,
and exercise caution when heeding its recommendations. A threshold
value is at least a useful starting point to start a search, and determining a sane initial value can greatly increase the ease of use of a plagiarism detection tool.

However, the task of locating a good initial threshold has received no attention
in the literature, and is therefore left completely to the personal decision of
the grader. The following example illustrates the problems raised by this issue.
A grader is asked to locate cases of plagiarism within a corpus of size 5. There
will be $\binom{5}{2}=12$ pairwise distances, say, 0.1, 0.15, 0.3, 0.6, 0.6,
0.62, 0.62, 0.64, 0.64, 0.65. It seems intuitive to flag 0.1 and 0.15 as
surprisingly small when compared to the rest; but how should 0.3 be considered?
The example may be driven further: assume now that the distribution of the above
distances is known to be uniform between 0 and 1: would the grader still flag
0.1 and 0.15 as surprising?
probably not, because those distances are fairly probable within a uniform
distribution. With no prior assumption about the mechanism which generated the
data, detection skills rely too much in the subjectivity of the grader.

Under certain conditions, it is possible to quantify the `amount of surprise'
presented by a given value within a sample. This problem is
completely equivalent to the one of finding \emph{outliers}, a classical problem
in statistical data analysis. Quoting Barnet and Lewis \cite[page~7]{Barnet94} 
\begin{quote} 
We shall define an outlier in a set of data to be an observation
(or subset of observations) which appears to be inconsistent with the remainder
of that set of data.
\end{quote}

% Later, the same authors provide a more precise description
% \cite[page~32]{Barnet94}
% \begin{quote}
% We have subjective doubts about the propriety of the outlying
% values both in relation to the specific data we have obtained and
% in relation to our initial views of an appropriate probability
% model to describe the generation of our data. Note how our
% feelings about the data may, in this respect, differ quite widely
% with different possible basic probability models.
% \end{quote}
%FIXME (MFreire): No me gusta la quote. Creo que no aclara demasiado... 
%FIXME' (MCebrian): Estoy de acuerdo, paso a quitarla.

% In the above lines, the authors state that it is not enough to observe a
% marked deviation of certain values from the remainder of the data; the
% deviation must also be unexplained according to the probability model of the
% mechanism that generated the data.

% Within a normal distribution, a large deviation from the mean would produce a
% stronger surprise than within a gamma distribution; in the case of a Cauchy
% distribution, still larger deviations would be expected. There is no point in
% performing a blind discrimination on the data without prior knowledge of the
% underlying probability model.

Those `surprisingly small
distances' are therefore equivalent to the term
\emph{lower outliers} as used in statistics. In other words, the set of
distances which should be flagged for further visual inspection during
plagiarism
detection  corresponds to what a reasonable statistical test will consider as
lower outliers within the full set of distances. As far as the authors are
aware, this is the very first application of outlier detection techniques to
plagiarism detection despite its natural analogy.

\subsubsection{Discordancy tests}

Having motivated the equivalence of both problems, the next step is to make use
of \emph{discordancy tests}, that is, statistical tests used to detect outliers
in a sample. 

More to the point, we are interested in designing discordancy test for two
scenarios:
\begin{itemize}
 \item \textbf{Scenario A} We want to detect outliers in the \emph{full ensemble
of distances} i.e. in the set $\{D(i,j) \ \text{for all submissions}
\ i,j\}$. The size of this set is $\binom{n}{2}$, where $n$ is the number of
submissions.

\item \textbf{Scenario B} We want to detect outliers in the \emph{individual
ensembles of distances}. Fixing the submission $k$, we want to detect
outliers in $\{D(k,j)\ \text{for all submissions} \ j \ne k\}$. If the
submission corpus has $n$ submissions, then there are $n$ different ensembles of
distances, one for each submission. The size of each individual ensemble is
therefore $n-1$.
\end{itemize}

Generally, the conditions for finding outliers in scenario A are
stronger than the ones in scenario B:
outliers in scenario A are outliers with respect to the full ensemble of
distances, while outliers in scenario B are outliers only with respect to
certain individual ensembles they belong to. The choice between one and
the other depends on the level of deterrence desired by the professor.

Once an scenario is chosen, discordancy tests are
designed as follows: the $n-k$ largest distances $x_n \ge x_{n-1} \ge
\ldots,x_{n-k+1}$ are assumed to originate from non-plagiarized pairs of
submission with an underlying probability model $F$. Meanwhile, the $k$ smaller
$x_k \ge x_{k-1} \ge \ldots \ge x_1$ are assumed to originate from a set of
plagiarized pairs with underlying probability model $G$. Of course, $k$ is
unknown to the grader.

\subsubsection{Hampel identifier}

There is strong statistical evidence that the probability distribution
for modelling in absence of plagiarism is the
normal distribution, and that plagiarized distances tend to be on the left of
this distribution, but significantly separated. Plagiarism can then be
considered as a generational mechanism which contaminates the normal
distribution samples with (a few) low distances.

% In the last affirmation there is an important assumption which is
% worth to remark. We have examined the tendency the distances by building
% Q-Qlots. In this plot, we have displayed the distances independently of
% whether  they belong to plagiarized pairs or not, so these distances also
% appear in the plots. Thefore, why are we claiming that there is evidence for
% of normal  distribution in the absence of plagiarism if we have plotted both
% plagiarized and non-plagiarized distances?
% 
% The key concept for understanding claim is the following: assume we have $n$
% total submissions, $k$ of them are plagiarism. In this case there are, on the
% one side $\binom{n-k}{2}$ non-plagiarized pairwise distances, those calculated
% between the $n-k$ `original' assigments. On the other hand, each plagiarism
% has one plagiarized distance and $n-2$ non-plagiarized distances, becase
% this is plagiarizing from one single source. So in total we have
% $\binom{n-k}{2} + k(n-2)$ non plagiarized distances and $k$ plagiarized
% distances.
% 
% \begin{table}
%  \centering
% \begin{tabular}{|c|c|c|c|c|}
% k & 10 & 20 & 30 & 40 & 50 \\ \hline
% non-plag. dist. & 4985 & 
% plag. dist &  10 & 
%  \end{tabular}
% \end{tabular}
% 
% \end{table}

It is possible to use a discordancy test able to extract the main
(normal) tendency
of the sample and to generate a model to detect outliers. Distances that
are deviations from normality are not a problem if an adequate discordancy test
is chosen which is neither influenced by lower outliers (plagiarism) nor from
upper
outliers (anomalous distances). The normality discordancy test should not be
affected by outliers of either sign.

There are several discordancy tests in the literature that fulfill these
conditions \cite[chapt.~6]{Barnet94}. The \emph{Hampel identifier},
is maybe the most extensively studied (see \cite{hampel1985bpm}). Additionally,
there is empirical data proving that it outperforms other tests in many
applications \cite{wilcox2003acs,pearson2002opm}.

The Hampel identifier works as follows. Let $X_{(1)},X_{(2)},...,X_{(N)}$ be the
ordered distances $X_1,X_2,\ldots,X_N$. Let $M$ be the \emph{median} of the
sample, and $S$ be the \emph{median absolute deviation form the median} of the
sample.

The Hampel identifier, adapted to lower outliers, is a rule which
identifies as plagiarisms all distances of the sample X satisfying $(M-X)/S >
g(N,\alpha)$ , where the function $g(N,\alpha)$ serves for standardizing the
identifier in the following way (see \cite{davies1993imo}, p. 783,
standardization (4)):
\begin{align}
\text{Probability}(\text{no outliers in the sample}) & =\text{Probability}\left(
\frac{|X_{(N)}-M)|}{S} <g(N,\alpha) \right )=\\
& =1 - \alpha.
\end{align}
The function $g(N,\alpha)$ does not have an analytic form and is estimated in
\ac{} by means of a Montecarlo simulation\footnote{A Matlab implementation to
locate critical values of the Hampel identifier ($g(N,\alpha)$) has been made
available by the authors at
http://www.mathworks.com/matlabcentral/fileexchange/\\loadFile.do?objectId=14769
} .

This method can handle a large number of outliers, and is resistant
to the problems appreciated in the non-parametric approach. We have
incorporated
it into both the and Graph+Population visualization
 (scenario A, see figure \ref{hampelfull}) and the Individual visualization
Histograms (scenario B, see figure \ref{hampelind}). We use the
thresholds  $\alpha=0.01$ and $\alpha = 0.05$ as default values.

More experimental work is needed to determine optimal thresholding values
($\alpha$ values), and
how this is affected by aspects such as the programming language, the
size of source code or the type of submission in the corpus. Future lines in
this research are detailed in section \ref{conclusion}.

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{hampelfull} 
\caption[Use of the Hampel identifier to recommend thresholds for
plagiarism detection in the Graph+Histogram visualization.]
{Use of Hampel identifier to recommend two
thresholds ($\alpha=0.05$ and $0.01$) for plagiarism (outlier) detection
in the Graph+Histogram visualization (scenario A).}
\label{hampelfull}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{hampelind} 
\caption[Use of Hampel identifier to recommend thresholds for
plagiarism detection in the Individual Histogram visualization.]
{Use of Hampel identifier to recommend two
thresholds ($\alpha=0.05$ and $0.01$) for each Individual Histogram
visualization (scenario B).}
\label{hampelind}
\end{figure*}



==> substring.tex <==
\subsubsection{Infrequent substrings similarity distance}
\label{substring}

This test is based on the observation that plagiarized sources are likely to share substrings which are infrequent within the whole corpus. Therefore, shared, infrequent substrings can be considered a strong indicator of similarity.

%Code which has been provided by the course instructor is likely not to be infrequent, as are common idioms in the corresponding programming language. These would be ignored by the test. However, if substrings shared by a pair of submissions can not be found anywhere else in the corpus, it is reasonable to assume a common origin.

For instance, given submissions $A$ and $B$ within a corpus of submissions written in the \textsc{C} programming language, $A$ and $B$ will likely share the substring \verb|printf|, since this is a common \textsc{C} idiom. On the other hand, other constructs, such as misspellings in comments or identifiers, are much rarer, and when found only in $A$ and $B$, can be considered as indications of a common origin.

Based on this idea, the \textit{Infrequent Substrings} distance builds a data structure (a sort of \textit{Patricia} tree \cite{ptree}) that stores every substring within a minimum and maximum length. This data structure can be used to calculate a similarity distance as follows:

\begin{center}
$\text{dist\_substring}(A, B) =$  \begin{Large} $\frac{f_{AB}}{n} \times \frac{l_{AB}}{L_\text{max}}$ \end{Large}
\end{center}

where $f_{AB}$ stands for the frequency within the corpus of the most infrequent substring shared by $A$ and $B$, $n$ is the number of submissions within this corpus, $l_{AB}$ stands for the length of the most infrequent substring shared between $A$ and $B$, and $L_\text{max}$ is the maximum substring length considered. In other words, those couples of submissions that share a very rare and long substring receive very small distance values.

%The \textit{Substring} distance has already been used with promising results in \cite{benchmark}, demonstrating that it is a valuable alternative to other similarity distance tests. Moreover, this test's results can be used to highlight areas of identical (and, more important, infrequent between two submissions), making it potentially valuable during visual side-by-side similarity inspection.

==> token.tex <==
\subsubsection{Token counting similarity distance}
\label{token}

The token-counting test is an example of attribute-counting test \cite{joy1999ppa}, in the sense that it does not analyze a program's structure, centering instead on the distribution of certain structure-independent attributes. The main idea behind the test is that, if two submissions share a substantial amount of code, then the frequency of each fundamental token in both submissions will be similar.

A vector is built for each submission $A$, such that $\mathbf{v}_A = (t_0, ... t_n)$, where $t_i$ represents the number of occurrences of token $i$ in $A$'s source files. The euclidean distance between each pair of vectors, $\mathbf{v}_{A_j}$ and $\mathbf{v}_{A_k}$, is then used as a similarity measure between $A_j$ and $A_k$.

Since the general contract of a similarity test requires results to be normalized in the range $[0, 1]$, normalization is performed by normalizing both vectors before checking their distance. Therefore, 

\begin{equation}
    \text{dist\_token}(A, B) = 
	\frac{\mathbf{v}_A}{|\mathbf{v}_A|} \cdot
	\frac{\mathbf{v}_B}{|\mathbf{v}_B|} = 
	cos(\widehat{\mathbf{v}_A \mathbf{v}_B})
\end{equation}

This is the vector-space model distance used in typical information
retrieval applications, as described in
\cite{baezayates99modern}. %However, it is not robust when used with
			   %programming submissions, since it is
			   %trivial to convert from certain tokens to other, semantically equivalent constructions in a way that completely thwarts this similarity comparison. It should therefore be used only in conjunction with stronger tests, as support.

% However, it must be noted that this test is completely resistant to attempts to disguise plagiarism by any structural obfuscation attempts, since it is only the relative frequency of tokens that is taken into account, and not their location within the source code. For instance, refactoring a program into different sets of functions would have a very small impact on token distribution, and would therefore fail to mislead the token-counting test.

==> unused.tex <==

% Automatic circumvention, Loki
Developing a tool that can automatically circumvent a given plagiarism detection system while generating plausible code is far beyond the abilities and goals of the typical plagiarizer.
%FIXME - This is the approach in the Loki Challenge.

% and the rest is...
Although automated systems can not, by themselves, solve the problem of incentivating graders to perform due diligence to keep submissions reasonably plagiarism-free, they are a fundamental part of this effort. As mentioned above, clear guidelines on plagiarism detection and prevention can help to incentivate graders to ensure that submissions are reasonably plagiarism-free. From a technical point of view, plagiarism detection systems must be extremely easy to use if they are to be successfull.

% social problem from a lone-crusader perspective.
Whatever the threshold for considering a segment of code as ``plagiarized'', there will always be examples which do not fall clearly into the ``good'' or ``bad'' category. If penalties are too high, graders that are comfronted with such cases will choose to err on the side of safety and not apply any penalty at all. This is more likely if there are no clear guidelines, or if a majority of graders do not actively search for plagiarism, since graders usually prefer not to antagonize students or be perceived as zealots by their colleagues.

% tools can provide proof
Additionally, automated tools can provide objective evidence to support their recommendations, by demonstating that a number of constructs are unique to a given pair of submissions. This evidence would be hard to generate without such tools, and can be very helpful when confronting the students. Because of the objective nature of these tests (in the sense that all submissions in the corpus are treated as equals), graders can have a lower 

% On the Variance Subtest
% Corrected distances $\mathbf{D'}_{ab}$ are calculated as follows:
%
% \begin{equation}
%   \text{LO}(a, b) = \frac{max(\widehat{\mathbf{D}_b} -
%     \mathbf{D}_{ab},\ 0)}{\text{LSD}(b)}
% \end{equation}
% \begin{equation}
%   \text{OI}(a, b)  = 2^{-{\text{LO}(a, b) \cdot \text{LO}(b, a)}}
% \end{equation}
% \begin{equation}
%   \mathbf{D'}_{ab} = \text{OI}(a, b) \cdot k \  + \  \mathbf{D}_{ab} \cdot (1 - k)
% \end{equation}
%
% Where the left standard deviation of a row $x$, $\text{LSD}(\mathbf{D}_x)$, is defined as the standard deviation of a matrix row calculated exclusively using distances $\mathbf{D}_{xy}$ lower than the mean of $\mathbf{D}_x$, $\widehat{\mathbf{D}_x}$. LO stands for ``left outlierness'', and is used to calculate an ``outlierness index'', OI, which is symmetrical and always falls between 0 (clear outlier) and 1 (not at all an outlier). Finally, $k$ is a weighing factor, used to modify the weight of OI in the final computation.


% On the problem of generating good benchmarks
According to a personal communication by Mike Joy, author of \textsc{Sherlock}\cite{joy1999ppa},
\begin{quote}
I think you have identified a fundamental problem [existence of public benchmarks or well-established
testing procedures] with research into plagiarism detection. I know of no benchmarks or established testing procedures, and I suspect there can never be any (since the criteria for establishing a case of plagiarism will vary depending on time / institution / culture / tutor's instructions / type of document / technology available to students).
\end{quote}

It is very difficult to obtain real-life precision-vs.-recall data for academic plagiarism detection software, because it is impractical to perform manual analysis on more than a few dozen pairs of assignments, and students are understandably reluctant to collaborate. In such a test, it would also be difficult to replicate the conditions under which most plagiarism is performed -- plagiarists usually do not want to ``trick the system'', they want to get a passing grade with minimal effort. The ``minimal effort'' part of the problem is difficult to replicate, since, if the system is correctly built, low efforts imply much greater chances of detection.

Comparing the output of several systems side-by-side and checking where they agree or disagree. At best, this will show whether your algorithm performs better than others. However, since most systems use very crude visualization, such a comparison would have to be restricted to ranked lists. Such a comparison would only cover the similarity-distance algorithm, ignoring many of main factors that impact usability (and therefore effectiveness) of a plagiarism detection system.

Asking graduate students to attempt to plagiarize a program and avoid detection. However, given enough time, code can be made to be arbitrarily different while retaining functionality. Therefore, the available time would have to be strictly limited, and in the best case, the experiment would ``prove'' that none of the test subjects had managed to defeat the system in the allotted time.

Substitute the grad students by a program that generates 'plagiarized' versions of the original sources. However, humans and computers are very different in their strengths and weaknesses. A computer can trivially replace all instances of each identifier that occurs in a program with randomly-generated versions. However, a grader would immediately notice the ``artificial look'' of the result. To generate plagiarized versions, the plagiarizing program would have to contain exact instructions on what to manipulate and how to do it to retain a minimum of plausibility from a graders' point of view. This is no small feat.

Using grammar evolution on a population of programs and see if you can later reconstruct mutation and crossover operations. This is a variation of the above scenario, where the 'plagiarizing program' is substituted with suitable genetic operators. Although the results are interesting from a theoretical standpoint (passing this test proves that the system works reliably when comfronted with large populations of diverse programs, some of which are plagiarized), the corpus will still be far from the stated goal: real submissions, with actual attempts to deceive the system in minimal time.

% Better intro
The development of the World Wide Web and the associated abundance of accessible electronic documents has lead to a greater incidence of plagiarism. In the case of undergraduate students, educators are generally ill-equipped to face the technological challenges posed by plagiarism. Exact figures are unknown, since successful plagiarism is by definition not detected, but are believed to be high and growing \cite{clare2000cpt,irving2000pde}. Alexander Aitken, one of the leading experts in operating plagiarism detection software, asserted in a personal communication prior to 2001 that for any (USA) student corpus, 10\% of submissions are plagiarized \cite[p.~4]{culwin2001scp}.


% Causes for plagiarism: real thing too tough or muddy, unreasonable faculty expectations, student thinks it is ok.
Among the most usual causes for plagiarism, we may find the following:
\begin{itemize}
\item Low ethical and/or technical preparation of the students.
\item Ambiguity in assignments: poorly understood exercises are more
likely to suffer plagiarism.
\item Low clarity in the university's guidelines on student collaboration.
\item Bad course planning causing an excessive work load.
\end{itemize}
In this light, a plagiarism detection tool can be considered as a sanity check, to be used in the diagnosis of the relative health of the teaching environment. 


% From 'intro.tex'
Notable features of \ac{} include the following:

\begin{itemize}

\item Intuitive display of results, providing visualizations such as as graphs and different types of histograms, allows visual exploration of analysis results. From the visualizations, plagiarism suspects can be selected in order to perform detailed manual analysis.

\item Extraction/filtering utility designed to ease the initial task of preparing assignment submissions for analysis. Submission preprocessing would otherwise be a repetitive and error-prone task; this utility seeks to automate the process without being specific to any particular institution.

\item Implements a novel distance integration architecture, allowing similarity distance algorithms to be combined, compared and refined. Many distance algorithms found in the scientific literature on plagiarism detection are included, together with several others developed by our research group.

\item Incorporates a novel threshold recommendation system based on statistical outlier detection. Distances lower than this threshold are suggested for manual analysis, establishing an heuristic starting point to help grader's unveiling of plagiarism patterns.

\item Open Source code, featuring a modular design that allows easy customization of both algorithms and visualizations. \ac{} can therefore be analyzed, extended and adapted for any particular requirements.

\item Stand-alone platform-independent program which can be executed in any computer with a \textsc{Java} runtime environment. There is no need to send the submissions to a server in a different institution, avoiding privacy concerns. Furthermore, a desktop application can deliver interactive visualizations which would be difficult to perform online.

\item Intended to be a long-term supported tool by means of facilities such as version source-control system, bug-tracking record, forums and an updated website. Transition to Sourceforge or other Open Source collaborative software management portals is currently under study.

\end{itemize}


% From 'state.tex'
\begin{enumerate}
\item[1. Whitespace insensitivity:] Matches between source codes should be unaffected by such things as extra whitespace, capitalization, punctuation, variable and function names, etc. 

\item[2. Noise suppression:] Discovering short matches, such as the fact that the word `the' appears in two different documents, is uninteresting. Any match must be large enough to imply that the material has been copied and is not simply a common word or idiom of the language in which documents are written.

\item[3. Position independence:] Coarse-grained permutation of the contents of a document (e.g., scrambling the order of paragraphs) should not affect the set of discovered matches. Adding to a document should not affect the set of matches in the original portion of the new document. Removing part of a document should not affect the set of matches in the portion that remains.
All schemes that we know
\end{enumerate}


%from former "practical example" section
\subsection{Artificial submissions}

This benchmark\footnote{available at {http://www.ii.uam.es/{\textasciitilde}mcebrian/plagiarism-benchmark/}} is composed of 44 programs in \emph{APL} that seek to implement the function $\cos(\log x)$. Thirty of the 44 programs are \textit{original} programs, and were generated by totally independent evolutionary runs with different random seeds. Six of them are `mutational plagiarized programs', obtained by applying the mutation operator to one of the original programs. Finally, eight of them are `recombination plagiarized programs', which have been generated by merging two original programs by means of crossover evolutionary operators. To facilitate the task of identifying the source codes, the different generated  programs have been labeled as follows $P1, P2, \dots P30$. Mutational-plagiarized programs use labels in the form MP\textit{x} (where \textit{Px} is the original source), and recombination-plagiarized P\textit{x}RGP\textit{y} or P\textit{x}RFP\textit{y},
where \textit{Px} and \textit{Py} represent the original programs identifiers. A graph representing the relations and structure of this corpus is presented in figure \ref{graph}.

\begin{figure*}[t]
\centering
\begin{tabular}{ccc}
\includegraphics[width=.7\textwidth]{graph} 
\end{tabular}
\caption{Plagiarism dependence of the artificial benchmark. Round vertices stand for
original submissions, boxes for plagiarism using a single source,
rhomboids and octagons for the two different types of plagiarism that use
two sources. A black solid line between two submissions denotes that one
 is a plagiarism of the other, a red dashed lines denotes that one is
one of the sources for plagiarism of the other and a green dotted line
denotes that they are indirect copies, i.e. they share a common source of
plagiarism.}
\label{graph}
\end{figure*}

Given this set of submissions, we run an un-tokenized \textit{Zip} similarity distance, which produces results which can be analyzed using any of the visualizations discussed in Section \ref{design}. The first visualization corresponds to the row data (see fig. \ref{tableTab-Artificial}). This output is not very helpful to find suspects of plagiarism, since single values have no meaning for our purposes, unless they are examined under the perspective of the whole population. 

The second visualization is depicted in figure \ref{graphTab-Artificial}. The graph on the top of the figure represents relations between submissions; the histogram below the graph displays a shaded portion, which is controlled by a slider. The graph only displays distances that fall within this shaded portion, allowing a grader to concentrate only on the shortest distances between submissions.

\begin{figure*}[p]
\centering
\begin{tabular}{ccc}
\includegraphics[height=.35\textheight]{tableTab-Artificial} 
\end{tabular}
\caption{Test results visualized as a distance table.}
\label{tableTab-Artificial}
\end{figure*}

\begin{figure*}[p]
\centering
\begin{tabular}{ccc}
\includegraphics[height=.4\textheight]{graphTab-Artificial} 
\end{tabular}
\caption[Test results visualized as a graph]{Test results visualized as a graph, with a histogram reflecting the frequency of each distance (ranging from 0, most similar, to 1) and a horizontal slider, used to select the maximum distance that is used for inclusion in the graph: only pairs of  submissions with a distance lower than this threshold are included.}
\label{graphTab-Artificial}
\end{figure*}

The interaction between slider and graph is detailed in section \ref{graphicalaid}. The initial value for the threshold is obtained from the Hampel identifier, but the slider can be freely adjusted by the user. In this example, the recommendation of the Hampel identifier (0.33) will be followed (with 95\% significance), as displayed in figure \ref{graphTab-Artificial}. All mutational-plagiarized programs (MP5, MP10, MP15, MP20, MP25 and MP30), and recombination-plagiarized (P10RGP5, P14RFP7, P15RGP20, P15RFP20, P1RFP30, P20RGP15, P22RFP5 and P5RGP10) are displayed. The only original submission that appear, although they have clearly not been copied or plagiarized, are P13, P14 and P18. It must be noted that two submissions can be very similar by arbitrary reasons, specially if the assignment is small and simple as in this case with
the function $\cos(\log x)$.

Although the graph visualization is already very useful to detect suspicious submissions, \ac{} provides a third output, depicted in figure \ref{indivHistogramsTab-Artificial}, which can improve our analysis. This output corresponds to the \emph{hue histograms} described in section \ref{graphicalaid}. The histogram for each row corresponds to distances between the row's submission and all others. This individual view provides a different perspective, from which new suspects can be found and others dismissed.

Certain conspicuous cases can be easily located. For instance, the lowest similarity distance value within the P25 histogram corresponds to its plagiarized sibling MP25; and is also clearly \textit{outside} the distribution of other distances. The same applies to P15, whose plagiarized siblings MP15 and P15RGP20 also exhibit low values. Large gaps are found within the individual histogram for P25 between MP25 and all other distances. The same large gap can be found in P15's individual histogram between distances for plagiarized siblings (MP15, P15RGP20) and those corresponding to all other programs. The meaning and relevance of these gaps is discussed in section \ref{hist_viz}.

\begin{figure*}[t]
\centering
\begin{tabular}{ccc}
\includegraphics[width=\textwidth]{indivHistogramsTab-Artificial} 
\end{tabular}
\caption[Test results visualized as individual histograms]{Test results visualized as individual histograms. Each row represents a color-coded histogram (blue is low, red is high) of the frequency with which other submissions have presented a given similarity to this one. Unexpected gaps in the leftmost side of the histogram suggest existence of plagiarism}
\label{indivHistogramsTab-Artificial}
\end{figure*}


==> variance.tex <==
% \subsubsection{Variance similarity distance}
\label{var_test}

The variance distance is a refinement on other tests, because it does not
compute a similarity directly from the source code of submissions. Instead, it
refines a distance matrix in an attempt to assign higher similarities to
``left-most'' outliers within individual distributions (see section
\ref{hist_viz}).

The intuitive goal is, when refining the distance between submissions, to give lower distances to submissions that appear as a ``left-most spike'' in each other's individual histograms. In a more formal characterization, let $A$ be a submission and $\mathbf{D}_A$ the set of distances from $A$ to all other submissions $X_{i}$, as found in a distance matrix $\textbf{D}$:

\begin{equation}
 \mathbf{D}_A = {\textbf{D}_{AX_1}, ..., \textbf{D}_{AX_n}}
\end{equation}

That is, $\mathbf{D}_A$ is a row from the distance matrix $\mathbf{D}$ that is to be refined as a result of running this test.

Let $B$, another submission, have an individual distribution $\mathbf{D}_B$. If $\mathbf{D}_{AB}$ is a left-most outlier (that is, is uncommonly low) in both $\mathbf{D}_A$ and $\mathbf{D}_B$, then there is a strong case for $A$ and $B$ to have much in common, regardless of the actual value of $\mathbf{D}_{AB}$ within the global distribution of distances (which may be moderate enough as to not currently arouse suspicion).

Since we are only interested in \emph{left-most outliers} (uncommonly low distances within a distribution), outliers to the right should not be considered. Therefore, our calculations substitute classical standard deviations of a distribution $\mathbf{D}_X$ for \emph{left standard deviations}, or $\text{LSD}(\mathbf{D}_X)$, defined as the standard deviation calculated exclusively using those distances $\mathbf{D}_{XY}$ such that $\mathbf{D}_{XY} < \widehat{\mathbf{D}_X}$, that is, lower than the mean of $\mathbf{D}_X$. Distances greater than the mean do not contribute towards the $\text{LSD}$.

The following metric is used to determine the \emph{outlierlyness} of $A$ in $B$:
\begin{equation}
    \text{out}(A, B) = \frac{max(\widehat{\mathbf{D}_B} - 
	\mathbf{D}_{AB},\ 0)}{\text{LSD}(B)}
\end{equation}
That is, the degree in which $A$ is a left-most outlier of $\mathbf{D}_B$ is 0 if $A$'s distance is greater than $\mathbf{D}_B$'s mean, and positive and proportional to the number of left-most standard deviations of the difference otherwise.

Using this definition, the degree of \emph{outlier importance} that we are willing to attribute to this fact is expressed by
\begin{equation}
    \text{OI}(A, B) = 2^{-{\text{out}(A, B) \cdot \text{out}(B, A)}}
\end{equation}

This exhibits the desirable traits of being symmetric ($\text{OI}(A, B) = \text{OI}(B, A)$), and bounded in the interval $]0, 1]$, since $\text{OI}(A, B) = 1$ when $\text{out}(A, B)$ or $\text{out}(B, A)$ are zero, and $\simeq 0$ when both are relatively high. The outlier importance can then be factored into a \emph{corrected distance} $\mathbf{D'}$ with a weighing constant $k_{oi}$:
\begin{equation}
    \mathbf{D'}_{AB} = OI(A, B) \cdot k_{oi} \  + \  \mathbf{D}_{AB} \cdot (1 - k_{oi})
\end{equation}

A value of $0.4$ for the outlier-importance constant $k_{oi}$ has proven useful in our experiments, and is currently the default value when the ``previous test'' $\mathbf{D}$ is a compression test. Once the compression test's results are refined with this test, the end effect on a histogram display is that gaps are enlarged, causing a few distances to become lower, and therefore ``uncovering'' previously hidden similarities between submissions.

\label{variance}

==> zip.tex <==
\subsubsection{Compression similarity distance}
\label{zip}

A natural measure of similarity is based on the observation that two strings $p$ and $q$ are similar if the basic blocks of $p$ are in $q$ and vice versa. String $p$ can be described by referencing the blocks belonging to $q$. If both strings are indeed similar, the description of $p$ using that of $q$ will be very simple.

This is essentially how a file compressor would operate on the
concatenated $pq$ sequence: the compressor would attempt to eliminate
redundant information from the merged sequence; if information from
$p$ is present in $q$, or vice-versa, the compressed size of $pq$,
$C(pq)$, will be smaller than $C(p) + C(q)$, since part of the
information contained in $p$ can be described by referencing suitable
blocks of $q$. This similarity measure was formalized by Rudi
Cilibrasi and Paul Vit\'anyi in \cite{cilibrasi2005cc} (with
\cite{saxon2000cpd} as a precursor), giving rise to the concept of
\emph{normalized compression distance} (NCD), based on the use of
compressors to provide a measures of the similarity between
sequences. This distance is defined as follows, and may then be used
to cluster documents made of strings.

\begin{equation}
\text{NCD}\left(p,q\right)=\frac{C\left(pq\right)-\min\left\{
C\left(p\right),C\left(q\right)\right\} }{\max\left\{
C\left(p\right),C\left(q\right)\right\}}
\label{model0}
\end{equation}
where $pq$ is the concatenation of strings $p$ and $q$, and $C(x)$  denotes the length of the text $x$ compressed using some compression algorithm which asymptotically reaches the true entropy of $x$ as the length of $x$ tends to infinity.

This idea is very powerful, because it can be applied in the same way to any type of sequence, be it music, text, or genetic data. There is no need to use specific features of sequences. The distance from sequence $p$ to sequence $q$ is simply a measure of the difficulty of using $p$ describe $q$ and vice versa.

%The first proposal to use this similarity distance for plagiarism detection can be found in \cite{saxon2000cpd}; however, it was not rigorously studied until the development of the \textsc{SID} engine (available at http://genome.math.uwaterloo.ca/SID/), experimentally demonstrating that the use of NCD as a text similarity distance within a plagiarism detection tool has advantages over other similarity distances \cite{SID}.

%NCD has been incorporated into \ac{} in two flavors: the \emph{Zip} test operateson tokenized source code (and is therefore dependent on the availability of a suitable parser) while the \emph{Gross Zip} distance operates on raw source code. The latter is specially useful when analyzing code written in programming languages for which it is difficult to obtain a parser. In both cases, compression is done by means of the standard \textsc{Java} compression library using the classical Lempel-Ziv algorithm \cite{ziv1977uas}.
